Quantifying Technical Debt: A Systematic Mapping Study and a Conceptual Model

To effectively manage Technical Debt (TD), we need reliable means to quantify it. We conducted a Systematic Mapping Study (SMS) where we identified TD quantification approaches that focus on different aspects of TD. Some approaches base the quantification on the identification of smells, some quantify the Return on Investment (ROI) of refactoring, some compare an ideal state with the current state of a software in terms of the software quality, and some compare alternative development paths to reduce TD. It is unclear if these approaches are quantifying the same thing and if they support similar or different decisions regarding TD Management (TDM). This creates the problem of not being able to effectively compare and evaluate approaches. To solve this problem, we developed a novel conceptual model, the Technical Debt Quantification Model (TDQM), that captures the important concepts related to TD quantification and illustrates the relationships between them. TDQM can represent varied TD quantification approaches via a common uniform representation, the TDQM Approach Comparison Matrix, that allows performing useful comparisons and evaluations between approaches. This paper reports on the mapping study, the development of TDQM, and on applying TDQM to compare and evaluate TD quantification approaches.

==> Tables/SMS_Table.tex <==
\begin{table}[t]
\centering
\begin{tabularx}{\textwidth}{l|l} 
%	\textbf{Type of TD} & \textbf{Num of Primary Studies} \\
		\midrule
    \emph{\textbf{SMS Iteration 1 --- Studies from 2010 - 2020}} &\\
		\midrule
	Defect & 4\\
    Documentation & 1\\
    Requirements & 1\\
    SATD & 2\\
    Scalability & 1\\
    Security & 2\\
    Service & 4\\
    Social & 1\\
    Sustainability & 1\\
    Compliance & 1\\
    Elasticity & 1\\
    Normalization & 1\\
    TD in BPMN & 1\\
    TD in ML & 1\\
    TD in Model Transfermation Languages & 1\\
    TD Related to DB Schemas & 1\\
    Temporal Adaption & 1\\
		\midrule
	\emph{Architecture} & 22\\
	\emph{Design} & 7\\
	\emph{Code} & 11\\
	\emph{Code and Architecture} & 3\\
	\emph{General} & 30\\
		\midrule
	\emph{Total} num of Studies for \emph{All types of TD} & 113\\
	    \midrule
	\emph{Total} num of Studies for \emph{Code related types of TD} & 73\\
		\midrule
	\emph{Unique quantification approaches} after grouping together related case studies \\for \emph{Code related types of TD} & 43\\
		\midrule
	\emph{\textbf{SMS Iteration 2 --- Studies from 2020 - 2022}} &\\
		\midrule
	Defect & 1\\
    Security & 1\\
    Normalization & 1\\
		\midrule
	\emph{Architecture} & 3\\
	\emph{Design} & 1\\
	\emph{Code} & 8\\
	\emph{General} & 1\\
		\midrule
	\emph{Total} num of Studies for \emph{All types of TD} & 16\\
	    \midrule
	\emph{Total} num of Studies for \emph{Code related types of TD} & 13\\
		\midrule
	\emph{Unique quantification approaches} after grouping together related case studies \\for \emph{Code related types of TD} & 6\\
			\midrule
	\emph{Total Unique quantification approaches \textbf{from both SMS Iterations}}
	\\for \emph{Code related types of TD} & ${43 + 6 = 49}$ \\
	\\
\end{tabularx}
\caption{Derivation of Unique Quantification Approaches for \emph{Code related types of TD}}
\label{tab:typesoftd_SMS_it}
\end{table}


==> Tables/inclusion_exclusion_criteria.tex <==
\begin{table}[h]
\centering
\begin{tabularx}{\textwidth}{c | l} 
%Inclusion/ Exclusion Criteria & \\\toprule
	Inclusion Criteria & \\
	  	& I1 Discusses approaches quantifying TD\\
	  	& I2 Discusses quantifiable characteristics of TD\\
	  	& I3 Discusses units of measurement that could be used to quantify TD\\
	  	& I4 Discusses SW Metrics in relation to TDM\\
	  	& I5 Evaluates an approach quantifying TD\\
	  	\midrule
	 Exclusion Criteria & \\
	  	& E1 Not a primary study\\
	  	& E2 The paper has not been peer reviewed\\
	  	& E3 The paper is not in English\\
	  	& E4 Research is not directly related to Quantifying TD\\
	  	& E5 Full text is inaccessible\\
\end{tabularx}
\caption{Inclusion and Exclusion Criteria}
\label{tab:inclexcl}
\end{table}

==> Tables/number_of_primary_studies_according_to_type_of_td.tex <==
\begin{table}[h]
\centering
\begin{tabularx}{\textwidth}{l|l} 
%	\textbf{Type of TD} & \textbf{Num of Primary Studies} \\
		\midrule
    \multicolumn{2}{l}\emph{\textbf{SMS Iteration 1 --- Studies from 2011 - 2020}} \emph{--- 113 Primary Studies in Total}\\
		\midrule
	Defect & 4\\
    Documentation & 1\\
    Requirements & 1\\
    SATD & 2\\
    Scalability & 1\\
    Security & 2\\
    Service & 4\\
    Social & 1\\
    Sustainability & 1\\
    Compliance & 1\\
    Elasticity & 1\\
    Normalization & 1\\
    TD in BPMN & 1\\
    TD in ML & 1\\
    TD in Model Transfermation Languages & 1\\
    TD Related to DB Schemas & 1\\
    Temporal Adaption & 1\\
	\emph{Architecture} & 22\\
	\emph{Design} & 7\\
	\emph{Code} & 11\\
	\emph{Code and Architecture} & 3\\
	\emph{General (inferred as code-related)} & 30\\
				%\midrule
	%\emph{Total} num of Studies for \emph{All types of TD} & 113\\
			\midrule
	\multicolumn{2}{l}\emph{\textbf{SMS Iteration 2 --- Studies from 2020 - 2022}} \emph{--- 16 Primary Studies in Total}\\
		\midrule
	Defect & 1\\
    Security & 1\\
    Normalization & 1\\
	\emph{Architecture} & 3\\
	\emph{Design} & 1\\
	\emph{Code} & 8\\
	\emph{General (inferred as code-related)} & 1\\
		%\midrule
	%\emph{Total} num of Studies for \emph{All types of TD} & 16\\
	\\
\end{tabularx}
\caption{Number of Primary Studies according to Type of TD | Italicised items --- code related types of TD}
\label{tab:typesoftd}
\end{table}
